CogniVoice: Multimodal and Multilingual Fusion Networks for Mild Cognitive Impairment Assessment from Spontaneous Speech

Mild Cognitive Impairment (MCI) is a medical condition characterized by noticeable declines in memory and cognitive abilities, potentially affecting individual's daily activities. In this paper, we introduce CogniVoice, a novel multilingual and multimodal framework to detect MCI and estimate Mini-Mental State Examination (MMSE) scores by analyzing speech data and its textual transcriptions. The key component of CogniVoice is an ensemble multimodal and multilingual network based on ``Product of Experts'' that mitigates reliance on shortcut solutions. Using a comprehensive dataset containing both English and Chinese languages from TAUKADIAL challenge, CogniVoice outperforms the best performing baseline model on MCI classification and MMSE regression tasks by 2.8 and 4.1 points in F1 and RMSE respectively, and can effectively reduce the performance gap across different language groups by 0.7 points in F1.

==> 020related.tex <==
\section{Related Work}

Existing approaches to detecting MCI %rising from diseases like Alzheimer's and Dementia 
use both textual and speech features in monolingual settings. Our work differs from previous work as it focuses on multilingual settings, effective ensemble, and multimodal and multilingual features extraction.


\noindent \textbf{Speech-based Methods.} \cite{farzana2023towards} focuses on feature-based and instance-based domain adaption techniques for heterogeneous speech to overcome data sparsity and improve generalizability across diverse datasets for dementia detection. \cite{ustc2023} develops an approach for AD detection by fine-tuning several wav2vec2.0~\cite{baevski2020wav2vec} models on various frequency bands, and for MMSE score prediction by combining the eGeMAPS~\cite{eyben2015geneva} acoustic features with silence features. \cite{tamm2023cross} use 25-dimensional eGeMAPS~\cite{eyben2015geneva} features for solving the same problem. They split the speech sequence into ten segments, and then concatenate the features of the ten segments, along with patient metadata. They perform classification using a two-layer MLP with an attention mechanism. Furthermore, multi-linguality is achieved by adapting an English pre-trained model to the second language using few-shot learning. \cite{cahyawijaya23_interspeech} studies a closely related problem which is speech emotion recognition and its transferability across age groups and languages.

\noindent \textbf{Text-based Methods:} \cite{santos2017enriching} transform transcripts into complex structures modeled as the co-occurrence network with words as nodes enriched with words embeddings and adjacent words have an edge; and used graph properties like page rank, centrality, etc and linguistics features, Bag-Of-Words features for classifiers to detect MCI.\cite{duan_cda_2023} uses a contrastive learning method for augmentation to improve the detection of Alzheimer’s disease on a small dataset, where they obtain the negative examples by randomly deleting the proportion of text from the transcripts.\cite{gkoumas2023digital} aims to capture language coherence by learning temporal logical consistency of utterances in short transcribed narratives to capture disruptive turns indicative of cognitive disorders.
\cite{zanwar_what_2023} explores fusion strategies on feature, model, and task level to improve the detection of Explainable Mental  Disorder.

\noindent \textbf{Multi-modal Methods:} \cite{dawalatabad2022detecting} focuses on mitigating the influence of the examiner by using speaker discriminative features based on speech and text methods to detect Dementia from examiner-patient conversion data.\cite{pappagari2020using} uses speaker recognition and natural language processing techniques to detect Alzheimer's disease and assess its severity where they analyzed the models for both modalities, individually and together, to examine its complementary and also found that the use of silence segments of the speech files acts as a complementary feature.\cite{DBLP:conf/interspeech/BalagopalanERN20} uses text and speech techniques, to provide the comparison and contrast between the methods which use domain knowledge-based hand-crafted features that capture linguistic and acoustic characteristics, and the methods, which fine-tunes BiDirectional Encoder Representations from Transformer (BERT) based sequence classification models. \cite{chou2023toward} focuses on joint training of speech and text instead of just focusing on learning based on only speech or text or both. \cite{chen2023} solve the tasks of AD detection and MMSE prediction in the multi-lingual setting by using paralinguistic features from openSMILE~\cite{eyben2010opensmile} and speech features from XLSR-53~\cite{conneau2021unsupervised}.
 

% \cite{dawalatabad2022detecting} focuses on the Dementia from examiner-patient conversion data. Inspired by the other research which states that the examiner’s language can influence the impairment classification, this paper studies the effect of the influence on the impairment classification task. To mitigate the effect of the examiner’s influence in evaluating cognitive impairment, they proposed a step approach. Firstly, by including speaker discriminative features to perform speech-based speaker diarization (i.e. who spoke when) followed by a text-based language model to distinguish between the examiner and patient. Finally, in the third stage they employ text and speech-based models to detect cognitive impairment from the segments. Their approach works on mono-lingual speech and transcripts. Compare to \cite{dawalatabad2022detecting}, \cite{santos2017enriching} uses language and graph network. \cite{santos2017enriching} transform transcripts into complex structure modeled as the co-occurrence network  with each unique word representing a node and the words that are adjacent in the text are connected by an edge. Constructed complex network is  enriched  with word embeddings to better represent short texts produced in the neuropsychological assessments. Measurements obtained from the network e.g page rank, centrality etc. are then used as features along with Linguistic and Bag-Of-Words features for well-known classifiers to automatically detect MCI. \cite{farzana2023towards} focuses on feature-based and instance-based domain adaption techniques for  heterogeneous spoken language data to evaluate generalizability across diverse datasets for dementia detection.

% \cite{pappagari2020using} uses speaker recognition and natural language processing techniques to detect Alzheimer disease and access its severity where they analyzed the models for both modalities, individually and together, to examine its complementarity and also found that the use of  silence segments of the speech files acts as a complementary features. Similar to \cite{pappagari2020using},
% \cite{DBLP:conf/interspeech/BalagopalanERN20} uses text and speech techniques, to provides the comparison and contrast between two approaches: first, which uses domain knowledge-based hand-crafted features that captures linguistic and acoustic characteristics, and second, which fine-tunes BiDirectional Encoder Representations from Transformer (BERT) based sequence classification models. 
% Other research works which utilizes text and speech features includes  \cite{chou_toward_2023} 
